The role of magnetoelastic coupling and magnetic anisotropy in MnTiO$_3$

We report the thermodynamic properties studied by thermal expansion, magnetostriction, magnetisation, and specific heat measurements as well as the low-energy magnetic excitations of \mto\ and investigate how magneto-elastic coupling and magnetic anisotropy affect the evolution of long-range order and the magnetic phase diagram. Specifically, we utilise high-resolution capacitance dilatometry and antiferromagnetic resonance (AFMR) studies by means of high-frequency electron spin resonance (HF-ESR) spectroscopy. The role of anisotropy is reflected by spin-reorientation at $B_{\rm{SF}}$~$\simeq 6$~T and a corresponding sign change in $\partial T_{\rm N}/\partial B$. Analysis of the AFMR modes enables us to establish the zero-field excitation gap $\Delta$ as well as its temperature dependence. We derive the effective anisotropy field $B_\mathrm{A} = 0.16(1)$~T which predominately originates from out-of-plane nearest-neighbour dipole-dipole interactions. Despite the nearly fully quenched orbital moment, our data show pronounced thermal expansion and magnetostriction anomalies at $T_{\rm N}$ and $B_{\rm{SF}}$ , respectively, which allows the experimental determination of sizable uniaxial pressure dependencies, i.e., $\partial B_{\rm SF}/\partial p_{\rm c} = -0.20(2)$~T/GPa, $\partial T_{\rm N}/ \partial p_b = 0.69(12)$~K/GPa, and $\partial T_{\rm N}/ \partial p_c = -2.0(4)$~K/GPa. Notably, short-range magnetic order appears up to at least 3$T_{\rm N}$ , as indicated by anisotropic lattice distortion, the violation of a constant Gr\"uneisen behavior, and the presence of local magnetic fields detected by HF-ESR.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
